Enhancing Small Language Models for Cross-Lingual Generalized Zero-Shot Classification with Soft Prompt Tuning

In NLP, Zero-Shot Classification (ZSC) has become essential for enabling models to classify text into categories unseen during training, particularly in low-resource languages and domains where labeled data is scarce. While pretrained language models (PLMs) have shown promise in ZSC, they often rely on large training datasets or external knowledge, limiting their applicability in multilingual and low-resource scenarios. Recent approaches leveraging natural language prompts reduce the dependence on large training datasets but struggle to effectively incorporate available labeled data from related classification tasks, especially when these datasets originate from different languages or distributions. Moreover, existing prompt-based methods typically rely on manually crafted prompts in a specific language, limiting their adaptability and effectiveness in cross-lingual settings. To address these challenges, we introduce RoSPrompt, a lightweight and data-efficient approach for training soft prompts that enhance cross-lingual ZSC while ensuring robust generalization across data distribution shifts. RoSPrompt is designed for small multilingual PLMs, enabling them to leverage high-resource languages to improve performance in low-resource settings without requiring extensive fine-tuning or high computational costs. We evaluate our approach on multiple multilingual PLMs across datasets covering 106 languages, demonstrating strong cross-lingual transfer performance and robust generalization capabilities over unseen classes.

==> tables/mlsum.tex <==
\begin{table}[H]
    \centering
    \setlength{\tabcolsep}{3.8pt}
    \renewcommand{\arraystretch}{1.1}
    \begin{tabular}{p{0.4cm}|c|cccc}
        \textbf{} &  & \textbf{de} & \textbf{es} & \textbf{fr} & \textbf{ru} \\ \hline
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{XGLM}}} & \textbf{RoSPrompt} & \textbf{79.47} & \textbf{70.77} & \textbf{71.60} & \textbf{62.66} \\
         & NPPrompt & 56.30 & 48.83 & 43.92 & 42.97 \\ 
         & NPPrompt-t & 61.22 & 21.68 & 31.97 & 38.24 \\
         & SPT & 63.12 & 53.26 & 54.00 & 53.68 \\ \hline
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{mT0}}} & \textbf{RoSPrompt} & \textbf{65.24} & 50.58 & \textbf{48.00} & 45.22 \\
         & NPPrompt & 65.07 & 48.10 & 43.23 & 43.14 \\ 
         & NPPrompt-t & 59.51 & 43.36 & 31.33 & 26.80 \\
         & SPT & 64.64 & \textbf{52.81} & 47.32 & \textbf{45.92} \\ \hline
        \multirow{4}{*}{\rotatebox[origin=c]{90}{\textbf{XLM-R}}} & \textbf{RoSPrompt} & \textbf{81.77} & \textbf{65.46} & \textbf{60.66} & 53.39 \\
         & NPPrompt & 62.38 & 50.77 & 52.79 & \textbf{58.17} \\ 
         & NPPrompt-t & 72.95 & 41.89 & 38.18 & 48.37 \\
         & SPT & 69.00 & 57.83 & 50.40 & 49.59 \\ \hline
    \end{tabular}
    \caption{Comparison of accuracy scores on the \textbf{MLSUM} dataset between RoSPrompt and baselines.}
    \label{tab:mlsum}
\end{table}


==> tables/mtop_domain.tex <==
\begin{table*}[t!]
\centering
    \setlength{\tabcolsep}{8pt}
    \renewcommand{\arraystretch}{1.1}
\begin{tabular}{c|c|cccccc}
\textbf{Model} &  & \textbf{de} & \textbf{en} & \textbf{es} & \textbf{fr} & \textbf{hi} & \textbf{th} \\ \hline
\multirow{4}{*}{\textbf{XGLM}} & \textbf{RoSPrompt} & \textbf{54.99} & \textbf{64.31} & \textbf{58.95} & \textbf{55.38} & \textbf{56.47} & 47.59 \\
 & NPPrompt & 48.72 & 55.02 & 47.77 & 47.57 & 52.49 & \textbf{49.26} \\
 & NPPrompt-t & 26.63 & 55.02 & 42.03 & 19.14 & - & 33.27 \\
 & SPT & 30.52 & 31.98 & 32.51 & 30.98 & 28.69 & 29.46 \\ \hline
\multirow{4}{*}{\textbf{mT0}} & \textbf{RoSPrompt} & \textbf{47.65} & \textbf{53.23} & \textbf{51.48} & \textbf{48.21} & \textbf{49.42} & \textbf{46.28} \\
 & NPPrompt & 43.14 & 46.35 & 48.57 & 43.60 & 46.04 & 38.37 \\ 
 & NPPrompt-t & 33.14 & 46.35 & 33.36 & 7.02 & - & 39.89 \\
 & SPT & 46.22 & 52.31 & 47.87 & 44.19 & 44.42 & 42.98 \\ \hline
\multirow{4}{*}{\textbf{XLM-R}} & \textbf{RoSPrompt} & \textbf{55.64} & \textbf{63.93} & \textbf{54.79} & \textbf{52.91} & \textbf{62.25} & \textbf{53.28} \\
 & NPPrompt & 36.38 & 46.03 & 35.76 & 34.95 & 47.69 & 39.02 \\ 
 & NPPrompt-t & 35.25 & 46.03 & 35.29 & 28.47 & - & 47.05 \\
 & SPT & 39.10 & 43.75 & 35.29 & 36.35 & 40.04 & 37.55 \\ \hline
\end{tabular}
\caption{Comparison of accuracy scores on the \textbf{MTOP} dataset between RoSPrompt and baselines.}
\label{tab:mtop}
\end{table*}

==> tables/sib-200-all-long.tex <==
{
    \setlength{\tabcolsep}{4pt}
    \onecolumn
    \begin{longtable}{c|cccc|cccc|cccc}
              & \multicolumn{4}{c|}{\textbf{XGLM}}                                           & \multicolumn{4}{c|}{\textbf{mT0}}                                              & \multicolumn{4}{c}{\textbf{XLM-R}}                                            \\ \hline
     \rule{0pt}{63pt} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{NPPrompt-t}} & \rotatebox{75}{\textbf{SPT}} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{NPPrompt-t}} & \rotatebox{75}{\textbf{SPT}} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{NPPrompt-t}} & \rotatebox{75}{\textbf{SPT}}  \\ \hline
    \endfirsthead
    
    \hline
              & \multicolumn{4}{c|}{\textbf{XGLM}}                                           & \multicolumn{4}{c|}{\textbf{mT0}}                                              & \multicolumn{4}{c}{\textbf{XLM-R}}                                            \\ \hline
     \rule{0pt}{63pt} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{NPPrompt-t}} & \rotatebox{75}{\textbf{SPT}} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{NPPrompt-t}} & \rotatebox{75}{\textbf{SPT}} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{NPPrompt-t}} & \rotatebox{75}{\textbf{SPT}}   \\
    \hline
    \endhead
    
    %\hline
    %\multicolumn{13}{r}{{Continued on next page}} \\
    \endfoot
    
    %\hline
    \endlastfoot
    
    % Your table data here, as before.
    afr\_Latn             &                &                     &                        &                          & 74.02          & 63.24              & 62.75                 & \textbf{74.39}          & \textbf{69.85} & 62.75              & 38.73                 & 59.07                   \\
als\_Latn             &                &                     &                        &                          & \textbf{75.37} & 62.75              & 56.86                 & 70.47                   & \textbf{69.24} & 65.69              & 24.02                 & 61.15                   \\
amh\_Ethi             &                &                     &                        &                          & \textbf{64.71} & 55.39              & -                     & 63.11                   & \textbf{65.56} & 59.80              & -                     & 62.38                   \\
arb\_Arab             & \textbf{69.12} & 60.78               & 53.92                  & 59.19                    & \textbf{71.69} & 62.25              & 64.71                 & 71.08                   & \textbf{72.67} & 69.61              & 55.39                 & 71.69                   \\
asm\_Beng             &                &                     &                        &                          &                &                    &                       &                         & \textbf{72.30} & 62.75              & -                     & 59.31                   \\
azb\_Arab             &                &                     &                        &                          & \textbf{65.07} & 54.41              & -                     & 58.58                   & \textbf{59.80} & 57.35              & -                     & 49.02                   \\
azj\_Latn             &                &                     &                        &                          & \textbf{75.37} & 63.24              & -                     & 69.73                   & 67.52          & \textbf{69.61}     & -                     & 67.16                   \\
bel\_Cyrl             &                &                     &                        &                          & \textbf{74.02} & 62.75              & 60.29                 & 69.36                   & \textbf{67.89} & 64.71              & 44.61                 & 66.67                   \\
ben\_Beng             & \textbf{69.36} & 61.27               & 61.27                  & 59.44                    & \textbf{72.30} & 57.35              & -                     & 69.85                   & \textbf{67.28} & 64.22              & -                     & 59.07                   \\
bos\_Latn             &                &                     &                        &                          &                &                    &                       &                         & \textbf{68.14} & 64.71              & 60.29                 & 58.70                   \\
bul\_Cyrl             & \textbf{69.49} & 63.73               & 57.35                  & 63.73                    & \textbf{77.45} & 63.24              & 55.88                 & 74.02                   & \textbf{68.26} & 66.18              & 59.80                 & 67.77                   \\
cat\_Latn             & \textbf{71.81} & 65.69               & 59.80                  & 59.19                    & \textbf{79.90} & 65.20              & 51.47                 & 71.32                   & \textbf{69.61} & 64.71              & 59.31                 & 67.77                   \\
ceb\_Latn             &                &                     &                        &                          & \textbf{69.12} & 61.27              & 54.41                 & \textbf{69.12}          &                &                    &                       &                         \\
ces\_Latn             &                &                     &                        &                          & \textbf{75.25} & 62.25              & 50.98                 & 71.81                   & \textbf{65.93} & 64.71              & 53.92                 & 64.83                   \\
cym\_Latn             &                &                     &                        &                          & \textbf{63.97} & 55.88              & 32.84                 & 63.48                   & \textbf{65.69} & 59.80              & 46.57                 & 59.19                   \\
dan\_Latn             &                &                     &                        &                          & \textbf{73.77} & 64.22              & 61.76                 & 72.06                   & \textbf{69.00} & 67.16              & 38.24                 & 64.22                   \\
deu\_Latn             & \textbf{70.22} & 62.25               & 48.04                  & 66.91                    & \textbf{75.12} & 66.18              & 62.25                 & 72.55                   & \textbf{69.36} & 68.14              & 50.49                 & 64.34                   \\
ell\_Grek             & \textbf{69.36} & 57.84               & 52.45                  & 62.75                    & \textbf{73.65} & 58.82              & 65.20                 & 69.49                   & 69.12          & \textbf{70.10}     & 47.06                 & 64.83                   \\
eng\_Latn             & \textbf{73.53} & 63.73               & 63.73                  & 69.00                    & \textbf{79.41} & 65.20              & 65.20                 & 73.53                   & \textbf{68.01} & 61.76              & 61.76                 & 52.33                   \\
epo\_Latn             &                &                     &                        &                          & \textbf{77.08} & 67.16              & 40.20                 & 73.04                   & \textbf{67.65} & 67.16              & 20.59                 & 59.44                   \\
est\_Latn             & \textbf{69.36} & 61.76               & 22.55                  & 65.56                    & \textbf{73.28} & 66.18              & 45.59                 & 72.30                   & \textbf{69.73} & 66.18              & 47.06                 & 58.21                   \\
eus\_Latn             & \textbf{71.20} & 63.73               & -                      & 60.17                    & \textbf{74.51} & 63.73              & -                     & 74.02                   & \textbf{65.81} & 58.82              & -                     & 58.33                   \\
fin\_Latn             & \textbf{73.65} & 62.75               & 58.82                  & 67.52                    & \textbf{72.92} & 62.25              & 52.45                 & 67.28                   & \textbf{71.45} & 66.18              & 59.31                 & 60.17                   \\
fra\_Latn             & \textbf{71.08} & 58.33               & 36.76                  & 60.05                    & \textbf{77.70} & 64.22              & 58.33                 & 70.71                   & \textbf{66.18} & 65.20              & 31.86                 & 60.17                   \\
gaz\_Latn             &                &                     &                        &                          &                &                    &                       &                         & \textbf{44.24} & 35.29              & 29.41                 & 38.48                   \\
gla\_Latn             &                &                     &                        &                          & \textbf{60.42} & 48.53              & 38.24                 & 56.13                   & \textbf{59.19} & 54.90              & 41.67                 & 53.19                   \\
gle\_Latn             &                &                     &                        &                          & 69.00          & 60.78              & 29.90                 & \textbf{69.24}          & \textbf{63.60} & 57.84              & 44.61                 & 56.86                   \\
glg\_Latn             &                &                     &                        &                          & \textbf{76.47} & 67.65              & 47.55                 & \textbf{76.47}          & \textbf{68.75} & 64.71              & 52.45                 & 68.50                   \\
guj\_Gujr             &                &                     &                        &                          & \textbf{74.02} & 65.20              & -                     & 69.24                   & \textbf{68.26} & 60.29              & -                     & 64.09                   \\
hat\_Latn             & \textbf{65.81} & 59.80               & 62.25                  & 48.41                    & \textbf{69.73} & 55.39              & 40.69                 & 67.40                   &                &                    &                       &                         \\
hau\_Latn             &                &                     &                        &                          & 60.91          & 51.47              & 42.65                 & \textbf{61.64}          & \textbf{60.54} & 59.31              & 45.59                 & 51.10                   \\
heb\_Hebr             &                &                     &                        &                          & \textbf{73.41} & 59.80              & 51.47                 & 68.26                   & \textbf{67.28} & 65.20              & 41.67                 & 64.83                   \\
hin\_Deva             & \textbf{67.89} & 62.25               & -                      & 58.09                    & \textbf{72.43} & 62.25              & -                     & 71.45                   & \textbf{71.20} & 65.69              & -                     & 65.56                   \\
hrv\_Latn             &                &                     &                        &                          &                &                    &                       &                         & \textbf{68.26} & 66.67              & 62.75                 & 58.09                   \\
hun\_Latn             &                &                     &                        &                          & \textbf{72.92} & 61.76              & -                     & 68.63                   & \textbf{69.98} & 64.71              & -                     & 53.55                   \\
hye\_Armn             &                &                     &                        &                          & \textbf{71.69} & 61.27              & 65.69                 & 66.54                   & \textbf{70.10} & 66.67              & 68.14                 & 63.60                   \\
ibo\_Latn             &                &                     &                        &                          & \textbf{71.45} & 62.25              & 55.88                 & 68.75                   &                &                    &                       &                         \\
ind\_Latn             & \textbf{73.04} & 59.31               & 63.73                  & 66.05                    & \textbf{75.61} & 67.16              & 57.84                 & 72.92                   & \textbf{71.69} & 67.16              & 63.73                 & 67.28                   \\
isl\_Latn             &                &                     &                        &                          & \textbf{70.96} & 61.27              & 53.92                 & 69.61                   & \textbf{67.77} & 67.65              & 39.22                 & 58.82                   \\
ita\_Latn             & \textbf{72.43} & 63.24               & 48.53                  & 63.24                    & \textbf{75.00} & 63.24              & 53.43                 & 73.16                   & \textbf{66.79} & 65.69              & 44.61                 & 63.73                   \\
jav\_Latn             &                &                     &                        &                          &                &                    &                       &                         & 66.54          & 60.78              & 51.96                 & \textbf{66.67}          \\
jpn\_Jpan             & \textbf{72.30} & 62.25               & -                      & 59.68                    & \textbf{75.49} & 62.75              & -                     & 72.18                   & \textbf{69.12} & 64.22              & -                     & 64.22                   \\
kan\_Knda             &                &                     &                        &                          & \textbf{72.92} & 62.25              & -                     & 68.75                   & 65.20          & \textbf{66.18}     & -                     & 66.05                   \\
kat\_Geor             &                &                     &                        &                          & \textbf{74.14} & 62.25              & 58.33                 & 72.30                   & \textbf{70.47} & 66.18              & 55.88                 & 65.93                   \\
kaz\_Cyrl             &                &                     &                        &                          & \textbf{76.96} & 63.24              & -                     & 71.20                   & \textbf{73.04} & 70.10              & -                     & 69.24                   \\
khk\_Cyrl             &                &                     &                        &                          & 69.73          & 58.33              & -                     & \textbf{69.85}          & \textbf{65.69} & 60.29              & -                     & 53.92                   \\
khm\_Khmr             &                &                     &                        &                          & \textbf{71.57} & 65.69              & 61.27                 & 70.71                   & 66.54          & \textbf{66.67}     & 52.45                 & 64.71                   \\
kir\_Cyrl             &                &                     &                        &                          & \textbf{70.83} & 60.78              & -                     & 69.00                   & \textbf{69.49} & 66.67              & -                     & 61.76                   \\
kmr\_Latn             &                &                     &                        &                          & 57.35          & 52.94              & -                     & \textbf{57.84}          & \textbf{64.09} & 59.31              & -                     & 61.40                   \\
kor\_Hang             & \textbf{68.38} & 60.78               & -                      & 62.99                    & \textbf{71.57} & 59.31              & -                     & 68.87                   & \textbf{69.00} & 63.24              & -                     & 62.62                   \\
lao\_Laoo             &                &                     &                        &                          & \textbf{74.39} & 65.69              & 61.76                 & 74.02                   & \textbf{68.63} & 61.27              & 60.78                 & 65.44                   \\
lit\_Latn             &                &                     &                        &                          & \textbf{74.02} & 64.71              & 64.71                 & 69.98                   & 66.05          & \textbf{67.65}     & 25.98                 & 57.35                   \\
ltz\_Latn             &                &                     &                        &                          & 66.42          & 55.88              & 44.61                 & \textbf{66.54}          &                &                    &                       &                         \\
lvs\_Latn             &                &                     &                        &                          & \textbf{74.26} & 61.76              & 47.55                 & 70.22                   & \textbf{69.12} & 62.75              & 24.51                 & 48.53                   \\
mal\_Mlym             &                &                     &                        &                          & \textbf{72.06} & 58.33              & -                     & 68.26                   & \textbf{70.10} & 66.18              & -                     & 64.83                   \\
mar\_Deva             &                &                     &                        &                          & \textbf{71.45} & 61.27              & -                     & 67.52                   & \textbf{67.03} & 61.27              & -                     & 57.60                   \\
mkd\_Cyrl             &                &                     &                        &                          & \textbf{76.47} & 60.78              & 63.73                 & 72.06                   & \textbf{70.83} & 61.27              & 59.80                 & 62.38                   \\
mlt\_Latn             &                &                     &                        &                          & \textbf{68.26} & 58.82              & 27.45                 & 66.18                   &                &                    &                       &                         \\
mri\_Latn             &                &                     &                        &                          & 56.13          & 47.06              & 26.47                 & \textbf{58.09}          &                &                    &                       &                         \\
mya\_Mymr             & \textbf{72.30} & 62.75               & -                      & 61.40                    & \textbf{71.32} & 58.33              & -                     & 70.71                   & \textbf{68.38} & 61.76              & -                     & \textbf{68.38}          \\
nld\_Latn             &                &                     &                        &                          & \textbf{76.35} & 63.73              & 66.18                 & 74.63                   & \textbf{70.34} & 68.14              & 51.96                 & 60.29                   \\
nno\_Latn             &                &                     &                        &                          & \textbf{74.14} & 63.73              & -                     & 69.24                   & \textbf{69.98} & 62.75              & -                     & 66.30                   \\
nob\_Latn             &                &                     &                        &                          & \textbf{75.25} & 62.75              & 58.82                 & 70.59                   & \textbf{70.96} & 64.71              & 38.73                 & 62.62                   \\
npi\_Deva             &                &                     &                        &                          & \textbf{73.04} & 62.25              & -                     & 70.34                   & \textbf{69.85} & 66.18              & -                     & 65.44                   \\
nya\_Latn             &                &                     &                        &                          & \textbf{70.59} & 61.76              & -                     & 69.24                   &                &                    &                       &                         \\
pan\_Guru             &                &                     &                        &                          & \textbf{72.30} & 61.76              & -                     & 71.94                   &                &                    &                       &                         \\
pbt\_Arab             &                &                     &                        &                          & 66.91          & 55.88              & -                     & \textbf{67.65}          & \textbf{65.07} & 62.75              & -                     & 62.62                   \\
pes\_Arab             &                &                     &                        &                          & \textbf{75.00} & 60.29              & -                     & 68.75                   & \textbf{68.75} & 65.69              & -                     & 61.03                   \\
plt\_Latn             &                &                     &                        &                          & \textbf{67.28} & 55.88              & -                     & 66.54                   & \textbf{62.99} & 54.90              & -                     & 48.04                   \\
pol\_Latn             &                &                     &                        &                          & \textbf{75.98} & 62.75              & 54.41                 & 74.14                   & \textbf{66.42} & 64.71              & 47.55                 & 64.95                   \\
por\_Latn             & \textbf{72.92} & 64.71               & 50.49                  & 66.18                    & \textbf{76.35} & 67.16              & 37.25                 & 74.02                   & \textbf{70.34} & 66.67              & 57.35                 & 68.63                   \\
quy\_Latn             & \textbf{45.71} & 44.12               & -                      & 32.48                    &                &                    &                       &                         &                &                    &                       &                         \\
ron\_Latn             &                &                     &                        &                          & 72.43          & 64.22              & 37.25                 & \textbf{75.86}          & \textbf{71.32} & 68.63              & 56.86                 & 62.01                   \\
rus\_Cyrl             & \textbf{70.22} & 60.78               & 57.84                  & 64.95                    & \textbf{75.49} & 63.73              & 61.27                 & 72.55                   & 68.75          & \textbf{69.12}     & 65.69                 & 67.28                   \\
san\_Deva             &                &                     &                        &                          &                &                    &                       &                         & \textbf{64.34} & 62.25              & -                     & 59.93                   \\
sin\_Sinh             &                &                     &                        &                          & \textbf{72.18} & 60.29              & -                     & 69.12                   & \textbf{68.14} & 62.25              & -                     & 60.05                   \\
slk\_Latn             &                &                     &                        &                          & \textbf{70.96} & 62.25              & 31.86                 & 69.61                   & 67.77          & \textbf{69.12}     & 65.20                 & 63.85                   \\
slv\_Latn             &                &                     &                        &                          & 72.43          & 62.25              & 52.94                 & \textbf{73.53}          & \textbf{65.93} & 64.71              & 61.27                 & 62.62                   \\
smo\_Latn             &                &                     &                        &                          & 60.91          & 50.49              & 49.51                 & \textbf{63.48}          &                &                    &                       &                         \\
sna\_Latn             &                &                     &                        &                          & \textbf{67.03} & 59.31              & 48.53                 & 64.71                   &                &                    &                       &                         \\
snd\_Arab             &                &                     &                        &                          & \textbf{65.32} & 58.33              & 43.63                 & 63.85                   & \textbf{67.40} & 58.82              & 16.67                 & 55.15                   \\
som\_Latn             &                &                     &                        &                          & 59.44          & 54.90              & 36.76                 & \textbf{60.05}          & \textbf{59.19} & 55.39              & 39.71                 & 52.21                   \\
sot\_Latn             &                &                     &                        &                          & \textbf{70.34} & 58.33              & 46.57                 & 67.40                   &                &                    &                       &                         \\
spa\_Latn             & \textbf{74.39} & 60.29               & 44.12                  & 55.88                    & \textbf{78.19} & 67.65              & 56.86                 & 74.02                   & \textbf{66.67} & 65.69              & 46.57                 & 68.50                   \\
srp\_Cyrl             &                &                     &                        &                          & \textbf{76.84} & 64.22              & 64.71                 & 71.08                   & \textbf{69.36} & 62.75              & 57.35                 & 59.56                   \\
sun\_Latn             &                &                     &                        &                          & \textbf{73.04} & 60.29              & 54.90                 & 70.83                   & \textbf{68.14} & 67.16              & 57.35                 & 67.40                   \\
swe\_Latn             &                &                     &                        &                          & \textbf{72.92} & 62.25              & 55.88                 & 70.96                   & \textbf{71.81} & 67.16              & 57.35                 & 66.67                   \\
swh\_Latn             & \textbf{65.32} & 61.76               & 58.82                  & 55.51                    & \textbf{71.69} & 61.76              & 49.51                 & 68.87                   & \textbf{65.69} & 62.75              & 50.00                 & 55.27                   \\
tam\_Taml             & \textbf{67.65} & 60.78               & -                      & 61.40                    & \textbf{76.10} & 62.75              & -                     & 71.32                   & \textbf{66.05} & 63.24              & -                     & 63.48                   \\
tel\_Telu             & \textbf{62.25} & 55.39               & -                      & 54.90                    & \textbf{75.12} & 63.24              & -                     & 71.94                   & \textbf{67.77} & 63.73              & -                     & 63.60                   \\
tgk\_Cyrl             &                &                     &                        &                          & \textbf{70.47} & 60.29              & 57.84                 & 66.79                   &                &                    &                       &                         \\
tgl\_Latn             &                &                     &                        &                          & \textbf{71.94} & 63.73              & 59.80                 & 68.63                   &                &                    &                       &                         \\
tha\_Thai             & \textbf{67.65} & 58.82               & 53.92                  & 59.31                    & \textbf{73.28} & 62.25              & 63.73                 & 70.96                   & \textbf{69.12} & 65.69              & 54.90                 & 68.87                   \\
tur\_Latn             & \textbf{72.55} & 62.25               & -                      & 60.42                    & \textbf{74.39} & 61.27              & -                     & 71.69                   & \textbf{67.89} & 65.20              & -                     & 63.11                   \\
uig\_Arab             &                &                     &                        &                          &                &                    &                       &                         & \textbf{67.16} & 62.25              & -                     & 59.93                   \\
ukr\_Cyrl             &                &                     &                        &                          & \textbf{73.65} & 62.75              & 63.24                 & 71.32                   & 67.89          & \textbf{69.61}     & 51.96                 & 66.79                   \\
urd\_Arab             & \textbf{67.65} & 56.86               & -                      & 55.27                    & \textbf{71.81} & 59.80              & -                     & 69.00                   & \textbf{70.83} & 61.76              & -                     & 65.69                   \\
uzn\_Latn             &                &                     &                        &                          & \textbf{74.63} & 63.24              & -                     & 69.49                   & \textbf{69.00} & 64.71              & -                     & 59.56                   \\
vie\_Latn             & \textbf{69.61} & 66.18               & 58.33                  & 59.31                    & \textbf{72.79} & 62.25              & 62.75                 & 70.34                   & 66.79          & \textbf{68.14}     & 54.90                 & 62.50                   \\
xho\_Latn             &                &                     &                        &                          & \textbf{69.36} & 61.27              & 50.49                 & 67.89                   & \textbf{52.82} & 50.49              & 26.47                 & 49.39                   \\
ydd\_Hebr             &                &                     &                        &                          & \textbf{60.66} & 53.43              & 43.14                 & 59.80                   & \textbf{62.25} & 51.47              & 30.39                 & 43.14                   \\
yor\_Latn             &                &                     &                        &                          & 55.88          & 49.51              & 40.69                 & \textbf{59.07}          &                &                    &                       &                         \\
zho\_Hans             & \textbf{73.53} & 54.90               & 44.61                  & 46.69                    & \textbf{77.21} & 63.24              & 58.33                 & 74.88                   & \textbf{68.87} & 63.24              & 56.86                 & 65.56                   \\
zho\_Hant             &                &                     &                        &                          & \textbf{74.14} & 65.69              & 61.76                 & 70.96                   & \textbf{70.22} & 66.18              & 54.90                 & 61.89                   \\
zsm\_Latn             &                &                     &                        &                          & \textbf{73.16} & 65.69              & 55.88                 & 69.36                   & \textbf{69.61} & 65.69              & 58.33                 & 60.42                   \\
zul\_Latn             &                &                     &                        &                          & \textbf{67.77} & 58.82              & 55.88                 & 65.44                   &                &                    &                       &                        \\ \hline
    \caption{Comparison of accuracy scores on the SIB-200 dataset between RoSPrompt and 3 different baselines across all supported languages.}\label{tab:sib-200-all}
    \end{longtable}
}

==> tables/sib-200-all.tex <==
\begin{table}
\small
\centering
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1}
\begin{tabular}{c|cc|cc|cc|}
 & \multicolumn{2}{c}{\textbf{XGLM}} & \multicolumn{2}{c}{\textbf{mT0}} & \multicolumn{2}{c}{\textbf{XLM-R}} \\ \hline \rule{0pt}{12ex}
 & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{RoSPrompt}} & \rotatebox{75}{\textbf{NPPrompt}} & \rotatebox{75}{\textbf{RoSPrompt}} \\ \hline
afr\_Latn &  & \textbf{} & 67.16 & \textbf{74.02} & 62.75 & \textbf{73.04} \\
als\_Latn &  & \textbf{} & 66.67 & \textbf{75.37} & 65.69 & \textbf{73.90} \\
amh\_Ethi &  & \textbf{} & 58.33 & \textbf{64.71} & 59.80 & \textbf{65.07} \\
arb\_Arab & 60.78 & \textbf{72.43} & 67.65 & \textbf{71.69} & 69.61 & \textbf{75.74} \\
asm\_Beng &  & \textbf{} &  & \textbf{} & 62.75 & \textbf{68.87} \\
azb\_Arab &  & \textbf{} & 52.94 & \textbf{65.07} & 57.35 & \textbf{63.24} \\
azj\_Latn &  & \textbf{} & 65.69 & \textbf{75.37} & 69.61 & \textbf{71.20} \\
bel\_Cyrl &  & \textbf{} & 64.22 & \textbf{74.02} & 64.71 & \textbf{71.69} \\
ben\_Beng & 61.27 & \textbf{71.32} & 63.73 & \textbf{72.30} & 64.22 & \textbf{67.65} \\
bos\_Latn &  & \textbf{} &  & \textbf{} & 64.71 & \textbf{70.22} \\
bul\_Cyrl & 63.73 & \textbf{71.94} & 66.67 & \textbf{77.45} & 66.18 & \textbf{72.30} \\
cat\_Latn & 65.69 & \textbf{75.74} & 70.10 & \textbf{79.90} & 64.71 & \textbf{74.02} \\
ceb\_Latn &  & \textbf{} & 64.71 & \textbf{69.12} &  & \textbf{} \\
ces\_Latn &  & \textbf{} & 70.59 & \textbf{75.25} & 64.71 & \textbf{70.22} \\
cym\_Latn &  & \textbf{} & 55.88 & \textbf{63.97} & 59.80 & \textbf{72.06} \\
dan\_Latn &  & \textbf{} & 67.65 & \textbf{73.77} & 67.16 & \textbf{72.79} \\
deu\_Latn & 62.25 & \textbf{73.28} & 69.12 & \textbf{75.12} & 68.14 & \textbf{71.57} \\
ell\_Grek & 57.84 & \textbf{74.51} & 67.16 & \textbf{73.65} & 70.10 & \textbf{74.02} \\
eng\_Latn & 63.73 & \textbf{76.84} & 70.59 & \textbf{79.41} & 61.76 & \textbf{72.43} \\
epo\_Latn &  & \textbf{} & 69.12 & \textbf{77.08} & 67.16 & \textbf{71.57} \\
est\_Latn & 61.76 & \textbf{72.79} & 67.16 & \textbf{73.28} & 66.18 & \textbf{71.32} \\
eus\_Latn & 63.73 & \textbf{67.65} & 68.14 & \textbf{74.51} & 58.82 & \textbf{70.34} \\
fin\_Latn & 62.75 & \textbf{76.72} & 67.16 & \textbf{72.92} & 66.18 & \textbf{73.65} \\
fra\_Latn & 58.33 & \textbf{75.61} & 66.67 & \textbf{77.70} & 65.20 & \textbf{70.71} \\
gaz\_Latn &  & \textbf{} &  & \textbf{} & 35.29 & \textbf{44.73} \\
gla\_Latn &  & \textbf{} & 55.88 & \textbf{60.42} & 54.90 & \textbf{60.05} \\
gle\_Latn &  & \textbf{} & 63.73 & \textbf{69.00} & 57.84 & \textbf{66.30} \\
glg\_Latn &  & \textbf{} & 69.12 & \textbf{76.47} & 64.71 & \textbf{74.14} \\
guj\_Gujr &  & \textbf{} & 65.69 & \textbf{74.02} & 60.29 & \textbf{69.73} \\
hat\_Latn & 59.80 & \textbf{71.57} & 61.27 & \textbf{69.73} &  & \textbf{} \\
hau\_Latn &  & \textbf{} & 56.37 & \textbf{60.91} & 59.31 & \textbf{63.11} \\
heb\_Hebr &  & \textbf{} & 63.24 & \textbf{73.41} & 65.20 & \textbf{72.67} \\
hin\_Deva & 62.25 & \textbf{74.14} & 66.18 & \textbf{72.43} & 65.69 & \textbf{73.77} \\
hrv\_Latn &  & \textbf{} &  & \textbf{} & 66.67 & \textbf{70.83} \\
hun\_Latn &  & \textbf{} & 64.22 & \textbf{72.92} & 64.71 & \textbf{71.08} \\
hye\_Armn &  & \textbf{} & 65.20 & \textbf{71.69} & 66.67 & \textbf{74.39} \\
ibo\_Latn &  & \textbf{} & 64.22 & \textbf{71.45} &  & \textbf{} \\
ind\_Latn & 59.31 & \textbf{76.23} & 71.08 & \textbf{75.61} & 67.16 & \textbf{75.74} \\
isl\_Latn &  & \textbf{} & 63.73 & \textbf{70.96} & 67.65 & \textbf{70.71} \\
ita\_Latn & 63.24 & \textbf{74.75} & 64.71 & \textbf{75.00} & 65.69 & \textbf{71.20} \\
jav\_Latn &  & \textbf{} &  & \textbf{} & 60.78 & \textbf{66.18} \\
jpn\_Jpan & 62.25 & \textbf{75.25} & 67.16 & \textbf{75.49} & 64.22 & \textbf{74.75} \\
kan\_Knda &  & \textbf{} & 65.69 & \textbf{72.92} & 66.18 & \textbf{70.22} \\
kat\_Geor &  & \textbf{} & 62.25 & \textbf{74.14} & 66.18 & \textbf{73.77} \\
kaz\_Cyrl &  & \textbf{} & 67.16 & \textbf{76.96} & 70.10 & \textbf{77.33} \\
khk\_Cyrl &  & \textbf{} & 61.27 & \textbf{69.73} & 60.29 & \textbf{69.00} \\
\multicolumn{2}{c}{khm\_Khmr} & \textbf{} & 64.71 & \textbf{71.57} & 66.67 & \textbf{69.98} \\
kir\_Cyrl &  & \textbf{} & 65.69 & \textbf{70.83} & 66.67 & \textbf{72.55} \\
kmr\_Latn &  & \textbf{} & 50.98 & \textbf{57.35} & 59.31 & \textbf{65.81} \\
kor\_Hang & 60.78 & \textbf{70.22} & 65.69 & \textbf{71.57} & 63.24 & \textbf{72.92} \\
lao\_Laoo &  & \textbf{} & 66.67 & \textbf{74.39} & 61.27 & \textbf{73.04} \\
lit\_Latn &  & \textbf{} & 66.67 & \textbf{74.02} & 67.65 & \textbf{70.22} \\
ltz\_Latn &  & \textbf{} & 59.80 & \textbf{66.42} &  & \textbf{} \\
lvs\_Latn &  & \textbf{} & 65.20 & \textbf{74.26} & 62.75 & \textbf{73.41} \\
mal\_Mlym &  & \textbf{} & 63.24 & \textbf{72.06} & 66.18 & \textbf{71.20} \\
mar\_Deva &  & \textbf{} & 63.24 & \textbf{71.45} & 61.27 & \textbf{67.89} \\
mkd\_Cyrl &  & \textbf{} & 66.67 & \textbf{76.47} & 61.27 & \textbf{72.30} \\
mlt\_Latn &  & \textbf{} & 61.76 & \textbf{68.26} &  & \textbf{} \\
mri\_Latn &  & \textbf{} & 50.49 & \textbf{56.13} &  & \textbf{} \\
mya\_Mymr & 62.75 & \textbf{77.33} & 64.71 & \textbf{71.32} & 61.76 & \textbf{70.34} \\
nld\_Latn &  & \textbf{} & 67.16 & \textbf{76.35} & 68.14 & \textbf{73.65} \\
nno\_Latn &  & \textbf{} & 69.12 & \textbf{74.14} & 62.75 & \textbf{71.94} \\
nob\_Latn &  & \textbf{} & 67.65 & \textbf{75.25} & 64.71 & \textbf{72.92} \\
npi\_Deva &  & \textbf{} & 66.18 & \textbf{73.04} & 66.18 & \textbf{74.14} \\
nya\_Latn &  & \textbf{} & 68.14 & \textbf{70.59} &  & \textbf{} \\
pan\_Guru &  & \textbf{} & 66.18 & \textbf{72.30} &  & \textbf{} \\
pbt\_Arab &  & \textbf{} & 57.35 & \textbf{66.91} & 62.75 & \textbf{68.87} \\
pes\_Arab &  & \textbf{} & 65.69 & \textbf{75.00} & 65.69 & \textbf{70.71} \\
plt\_Latn &  & \textbf{} & 60.78 & \textbf{67.28} & 54.90 & \textbf{63.24} \\
pol\_Latn &  & \textbf{} & 63.73 & \textbf{75.98} & 64.71 & \textbf{70.34} \\
por\_Latn & 64.71 & \textbf{77.33} & 69.61 & \textbf{76.35} & 66.67 & \textbf{74.14} \\
quy\_Latn & 44.12 & \textbf{48.16} &  & \textbf{} &  & \textbf{} \\
ron\_Latn &  & \textbf{} & 61.76 & \textbf{72.43} & 68.63 & \textbf{73.77} \\
rus\_Cyrl & 60.78 & \textbf{72.06} & 66.18 & \textbf{75.49} & 69.12 & \textbf{73.53} \\
san\_Deva &  & \textbf{} &  & \textbf{} & 62.25 & \textbf{66.54} \\
sin\_Sinh &  & \textbf{} & 63.73 & \textbf{72.18} & 62.25 & \textbf{70.22} \\
slk\_Latn &  & \textbf{} & 66.67 & \textbf{70.96} & 69.12 & \textbf{70.71} \\
slv\_Latn &  & \textbf{} & 65.20 & \textbf{72.43} & 64.71 & \textbf{70.71} \\
smo\_Latn &  & \textbf{} & 59.31 & \textbf{60.91} &  & \textbf{} \\
sna\_Latn &  & \textbf{} & 59.80 & \textbf{67.03} &  & \textbf{} \\
snd\_Arab &  & \textbf{} & 58.33 & \textbf{65.32} & 58.82 & \textbf{70.34} \\
som\_Latn &  & \textbf{} & 56.86 & \textbf{59.44} & 55.39 & \textbf{61.40} \\
sot\_Latn &  & \textbf{} & 63.73 & \textbf{70.34} &  & \textbf{} \\
spa\_Latn & 60.29 & \textbf{75.86} & 72.06 & \textbf{78.19} & 65.69 & \textbf{72.67} \\
srp\_Cyrl &  & \textbf{} & 68.63 & \textbf{76.84} & 62.75 & \textbf{73.65} \\
sun\_Latn &  & \textbf{} & 66.67 & \textbf{73.04} & 67.16 & \textbf{71.94} \\
swe\_Latn &  & \textbf{} & 65.69 & \textbf{72.92} & 67.16 & \textbf{74.39} \\
swh\_Latn & 61.76 & \textbf{66.67} & 65.20 & \textbf{71.69} & 62.75 & \textbf{68.50} \\
tam\_Taml & 60.78 & \textbf{73.16} & 65.20 & \textbf{76.10} & 63.24 & \textbf{71.08} \\
tel\_Telu & 55.39 & \textbf{70.83} & 66.67 & \textbf{75.12} & 63.73 & \textbf{69.73} \\
tgk\_Cyrl &  & \textbf{} & 65.69 & \textbf{70.47} &  & \textbf{} \\
tgl\_Latn &  & \textbf{} & 68.14 & \textbf{71.94} &  & \textbf{} \\
tha\_Thai & 58.82 & \textbf{72.67} & 66.67 & \textbf{73.28} & 65.69 & \textbf{73.41} \\
tur\_Latn & 62.25 & \textbf{72.79} & 67.16 & \textbf{74.39} & 65.20 & \textbf{69.36} \\
uig\_Arab &  & \textbf{} &  & \textbf{} & 62.25 & \textbf{68.14} \\
ukr\_Cyrl &  & \textbf{} & 64.71 & \textbf{73.65} & 69.61 & \textbf{72.43} \\
urd\_Arab & 56.86 & \textbf{70.34} & 61.27 & \textbf{71.81} & 61.76 & \textbf{73.28} \\
uzn\_Latn &  & \textbf{} & 66.67 & \textbf{74.63} & 64.71 & \textbf{69.24} \\
vie\_Latn & 66.18 & \textbf{74.26} & 68.63 & \textbf{72.79} & 68.14 & \textbf{71.20} \\
xho\_Latn &  & \textbf{} & 62.75 & \textbf{69.36} & 50.49 & \textbf{54.17} \\
ydd\_Hebr &  & \textbf{} & 50.49 & \textbf{60.66} & 51.47 & \textbf{62.25} \\
yor\_Latn &  & \textbf{} & 50.98 & \textbf{55.88} &  & \textbf{} \\
zho\_Hans & 54.90 & \textbf{77.45} & 70.59 & \textbf{77.21} & 63.24 & \textbf{73.90} \\
zho\_Hant &  & \textbf{} & 69.12 & \textbf{74.14} & 66.18 & \textbf{73.77} \\
zsm\_Latn &  & \textbf{} & 68.63 & \textbf{73.16} & 65.69 & \textbf{75.12} \\
zul\_Latn &  & \textbf{} & 64.22 & \textbf{67.77} &  & \\ 
\end{tabular}
\end{table}

==> tables/sib-200.tex <==
\begin{table*}[]
\centering
\small
\renewcommand{\arraystretch}{1.5}
\begin{tabular}{c|c|cccccccccc}
 &  & \textbf{ar} & \textbf{bn} & \textbf{bg} & \textbf{ca} & \textbf{de} & \textbf{el} & \textbf{en} & \textbf{et} & \textbf{eu} & \textbf{fi} \\ \hline
\multirow{2}{*}{XGLM} & RoSPrompt & \textbf{72.43} & \textbf{71.32} & \textbf{71.94} & \textbf{75.74} & \textbf{73.28} & \textbf{74.51} & \textbf{76.84} & \textbf{72.79} & \textbf{67.65} & \textbf{76.72} \\
 & Zhao et al. (2023) & 60.78 & 61.27 & 63.73 & 65.69 & 62.25 & 57.84 & 63.73 & 61.76 & 63.73 & 62.75 \\ \hline
\multirow{2}{*}{mT0} & RoSPrompt & \textbf{71.69} & \textbf{72.30} & \textbf{77.45} & \textbf{79.90} & \textbf{75.12} & \textbf{73.65} & \textbf{79.41} & \textbf{73.28} & \textbf{74.51} & \textbf{72.92} \\
 & Zhao et al. (2023) & 63.24 & 65.20 & 68.14 & 71.08 & 69.12 & 68.14 & 71.57 & 65.2 & 69.12 & 63.73 \\ \hline
\multirow{2}{*}{XLM-R} & RoSPrompt & \textbf{75.74} & \textbf{67.65} & \textbf{72.30} & \textbf{74.02} & \textbf{71.57} & \textbf{74.02} & \textbf{72.43} & \textbf{71.32} & \textbf{70.34} & \textbf{73.65} \\
 & Zhao et al. (2023) & 69.61 & 64.22 & 66.18 & 64.71 & 68.14 & 70.10 & 61.76 & 66.18 & 58.82 & 66.18 \\ \hline \hline
 &  & \textbf{fr} & \textbf{hi} & \textbf{id} & \textbf{it} & \textbf{ja} & \textbf{ko} & \textbf{my} & \textbf{pt} & \textbf{ru} & \textbf{es} \\ \hline
\multirow{2}{*}{XGLM} & RoSPrompt & \textbf{75.61} & \textbf{74.14} & \textbf{76.23} & \textbf{74.75} & \textbf{75.25} & \textbf{70.22} & \textbf{77.33} & \textbf{77.33} & \textbf{72.06} & \textbf{75.86} \\
 & Zhao et al. (2023) & 58.33 & 62.25 & 59.31 & 63.24 & 62.25 & 60.78 & 62.75 & 64.71 & 60.78 & 60.29 \\ \hline
\multirow{2}{*}{mT0} & RoSPrompt & \textbf{77.70} & \textbf{72.43} & \textbf{75.61} & \textbf{75.00} & \textbf{75.49} & \textbf{71.57} & \textbf{71.32} & \textbf{76.35} & \textbf{75.49} & \textbf{78.19} \\
 & Zhao et al. (2023) & 66.67 & 63.73 & 68.63 & 69.61 & 68.14 & 61.27 & 62.25 & 70.10 & 65.69 & 71.57 \\ \hline
\multirow{2}{*}{XLM-R} & RoSPrompt & \textbf{70.71} & \textbf{73.77} & \textbf{75.74} & \textbf{71.20} & \textbf{74.75} & \textbf{72.92} & \textbf{70.34} & \textbf{74.14} & \textbf{73.53} & \textbf{72.67} \\
 & Zhao et al. (2023) & 65.20 & 65.69 & 67.16 & 65.69 & 64.22 & 63.24 & 61.27 & 66.67 & 69.12 & 65.69 \\ \hline \hline
 &  & \textbf{sw} & \textbf{ta} & \textbf{te} & \textbf{th} & \textbf{tr} & \textbf{ur} & \textbf{vi} & \textbf{zh} &  &  \\ \cline{1-10}
\multirow{2}{*}{XGLM} & RoSPrompt & \textbf{66.67} & \textbf{73.16} & \textbf{70.83} & \textbf{72.67} & \textbf{72.79} & \textbf{70.34} & \textbf{74.26} & \textbf{77.45} &  &  \\
 & Zhao et al. (2023) & 61.76 & 60.78 & 55.39 & 58.82 & 62.25 & 56.86 & 66.18 & 54.90 &  &  \\ \cline{1-10}
\multirow{2}{*}{mT0} & RoSPrompt & \textbf{71.69} & \textbf{76.10} & \textbf{75.12} & \textbf{73.28} & \textbf{74.39} & \textbf{71.81} & \textbf{72.79} & \textbf{77.21} &  &  \\
 & Zhao et al. (2023) & 66.67 & 67.16 & 65.20 & 65.69 & 70.59 & 61.76 & 65.69 & 67.16 &  &  \\ \cline{1-10}
\multirow{2}{*}{XLM-R} & RoSPrompt & \textbf{68.50} & \textbf{71.08} & \textbf{69.73} & \textbf{73.41} & \textbf{69.36} & \textbf{73.28} & \textbf{71.20} & \textbf{73.90} &  &  \\
 & Zhao et al. (2023) & 62.75 & 63.73 & 64.22 & 65.69 & 65.20 & 61.76 & 68.14 & 63.24 &  &  \\ \cline{1-10}
\end{tabular}
\end{table*}
